Optimizing the Consumption of Spiking Neural Networks with Activity Regularization

Reducing energy consumption is a critical point for neural network models running on edge devices. In this regard, reducing the number of multiply-accumulate (MAC) operations of Deep Neural Networks (DNNs) running on edge hardware accelerators will reduce the energy consumption during inference. Spiking Neural Networks (SNNs) are an example of bio-inspired techniques that can further save energy by using binary activations, and avoid consuming energy when not spiking. The networks can be configured for equivalent accuracy on a task through DNN-to-SNN conversion frameworks but their conversion is based on rate coding therefore the synaptic operations can be high. In this work, we look into different techniques to enforce sparsity on the neural network activation maps and compare the effect of different training regularizers on the efficiency of the optimized DNNs and SNNs.

==> auc_table.tex <==

\begin{table*}[h!]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccc}
\hlineB{3}
\textbf{Architecture} & \textbf{L2} & \textbf{L1} & \textbf{L0.5} & \textbf{L0.01} & \textbf{H} & \textbf{Hs} \\
\hline
LeNet-5 & 0.9348 / 0.9432 & 0.9566 / 0.9606 & 0.9597 / 0.9653 & 0.7191 / 0.9298 & 0.7525 / 0.7663 & 0.7684 / 0.7740 \\
MLP & 0.9582 / 0.9652 & 0.9692 / 0.9764 & 0.9751 / 0.9755 & 0.9364 / 0.9663 & 0.9218 / 0.9286 & 0.9173 / 0.9228 \\
\hline
Average &  0.9465 / 0.9542 & 0.9629 / 0.9685 & \textbf{0.9674} / \textbf{0.9704} & 0.82775 / 0.94805 & 0.83715 / 0.84745 & 0.84285 / 0.774 \\
%Overall & 0.95035	& 0.9657 & \textbf{0.9689} & 0.8879 & 0.8423	& 0.808425 \\
\hlineB{3}
\end{tabular}
}
\caption{Area under the curve for both architecture. The values are formatted as (AUC(original) / AUC(smoothed)) }
\label{tab:auc}
\end{table*}

==> figure_eflops.tex <==
\begin{figure}[htb]

\begin{minipage}[b]{.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{images/Dense.png}}
%  \vspace{1.5cm}
  \centerline{(a) Dense layer}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{images/Conv.png}}
%  \vspace{1.5cm}
  \centerline{(b) 2D convolution layer}\medskip
\end{minipage}
%
\caption{Illustration of computation taking place for non-zero activations. Black dots represent zero-activated neurons, while the yellow dots are non-zero. (a) Dense layer. The number of multiply-adds executed equals the number of non-zeros neurons in layer $l_i$ times the number of outgoing connections. Green lines represent non-zero weights (b) 2D convolutional layer. In this example, the number of multiply-adds is proportional to the number of non-zeros neurons in layer $l_i$ and their contribution in the following layer. Here, all weights are considered to be equal to 1.}
\label{fig:eflops}
%
\end{figure}

==> res_table.tex <==
\begin{table*}[h]
\centering
\resizebox{1.0\linewidth}{!}{\begin{tabular}{lccccc}
\hlineB{3}
%\textbf{Regularization} & 
\textbf{$\lambda_{reg}$} & \textbf{Total Spikes}  & \textbf{EFLOPS} & \textbf{SynOps} & \textbf{Accuracy} & \textbf{SNN } \\

\hlineB{3}
MLP Baseline & 81787 & 68046 & 5349386 & 97.85\% & 97.66\% \\
\hline
  & \textbf{$\Delta$Spikes}  & \textbf{$\Delta$EFLOPS} & \textbf{$\Delta$SynOps} & \textbf{$\Delta$Accuracy} & \textbf{$\Delta$SNN } \\
\hline
L2 @ 5e-03 & 3.31x & 1.40x & 11.47x & -0.20\% & 0.00\%  \\
L1 @ 1e-03 & 8.04x & 1.42x & 22.15x & -0.20\% & -0.20\% \\
L0.5 @ 1e-03 & \textbf{12.35x} & 1.43x & \textbf{33.78x} & -0.20\% & 0.00\% \\
L0.01 @ 7e-03 & 6.01x & 1.40x & 11.85x & -0.59\% & -0.39\% \\
H @ 3e-03 & 2.02x & 1.02x & 2.83x & 0.00\% & 0.20\% \\
Hs @ 1e-05 & 1.93x & 1.02x & 2.82x & 0.20\% & 0.00\% \\
\hlineB{3}
LeNet-5 Baseline & 1131537  & 293642 & 60704434 & 99.02\% & 98.44\% \\
\hline
 & \textbf{$\Delta$Spikes}  & \textbf{$\Delta$EFLOPS} & \textbf{$\Delta$SynOps} & \textbf{$\Delta$Accuracy} & \textbf{$\Delta$SNN } \\
\hline
L2 @ 1e+00 & 5.68x & 4.07x & 10.02x & -0.20\% & 0.00\% \\
L1 @ 9e-04 & 6.43x & 3.54x & 10.32x & -0.20\% & -0.39\%  \\
L0.5 @ 7e-05 & \textbf{8.28x} & 4.00x & \textbf{10.85x} & 0.59\% & -0.39\% \\
L0.01 @ 7e-05 & 3.48x & 2.91x & 3.80x & 0.00\% & 0.39\% \\
H @ 6e-03 & 1.58x & 1.52x & 1.77x & 0.59\% & -0.20\% \\
Hs @ 1e-05 & 1.57x & 1.49x & 1.76x & -0.59\% & -0.39\% \\
\hlineB{3}
\end{tabular}}
\caption{Effect of regularization on the MLP and LeNet-5 architecture.} 
\label{tab:results}
\end{table*}
